Unbiasing Semantic Segmentation For Robot Perception using Synthetic Data Feature Transfer

Robot perception systems need to perform reliable image segmentation in real-time on noisy, raw perception data. State-of-the-art segmentation approaches use large CNN models and carefully constructed datasets; however, these models focus on accuracy at the cost of real-time inference. Furthermore, the standard semantic segmentation datasets are not large enough for training CNNs without augmentation and are not representative of noisy, uncurated robot perception data. We propose improving the performance of real-time segmentation frameworks on robot perception data by transferring features learned from synthetic segmentation data. We show that pretraining real-time segmentation architectures with synthetic segmentation data instead of ImageNet improves fine-tuning performance by reducing the bias learned in pretraining and closing the \textit{transfer gap} as a result. Our experiments show that our real-time robot perception models pretrained on synthetic data outperform those pretrained on ImageNet for every scale of fine-tuning data examined. Moreover, the degree to which synthetic pretraining outperforms ImageNet pretraining increases as the availability of robot data decreases, making our approach attractive for robotics domains where dataset collection is hard and/or expensive.

==> backup/old.tex <==
%% COMMENTED OUT CONTENT:

%% Abstract:
% The ability of a robot to reason about the geometry and semantics of its environment is fundamental to interactive robot behaviors, but often challenging due to perception frameworks that are trained on too little data or data not representative of the robot’s environment. In this work, we investigate the potential gains of using synthetic data to augment the training process of convolutional neural networks designed to enable real-time semantic segmentation for robots with limited real-world training data. We investigate the degree to which a larger amounts of data improves performance when training such a model, the relationship between the way a deep neural network is trained using multiple sources of synthetic segmentation data to pretrain standard segmentation datasets that apply to robotics and autonomous driving, and show that our method outperforms both training from scratch and standard data augmentation practices like pretraining on ImageNet. We show that synthetic data does continue to improve these models in spite of real-time model architectures having many fewer parameters than typical deep neural networks, and therefore hypothetically less representational power. Finally, we show how this approach generalizes to small purpose-built robot vision datasets on data acquired using an HRI robot.


%% Intro:
% In robotics and automation, the richest and most utilized type of sensing data is image data. this is because accurate perception of objects is crucial for fundamental robot behaviors such as object interaction and manipulation, semantic mapping, and obstacle avoidance.
 
% Segmentation is important for fine motion planning through obstacles, especially in cluttered environments, and physical robot interactions like grasping, push, and tool use tasks.  However, segmentation in robot vision is challenging because data from robot perception systems is \varun{limited,} noisy, unprocessed, and has very sparse supervision to help robots learn and adapt. 

% Historically, robots have depended on maintaining some expert domain knowledge to reason about objects in a complex scene, such as in \cite{pauwels2015simtrack}. This domain knowledge could take the form of a object models database that improved detection and tracking, or structuring the robot's environment in a known, static way. While these approaches work well for robots in structured environments where they only encounter a few known objects, these deterministic representations of the environment neither scale to large sets of objects and environments nor generalize well to new object instances. As a result, robots have been limited in their ability to function outside their research environments. \varun{This paragraph seems out of place. Maybe put it in the related work section?}

% Convolutional neural networks (CNNs), on the other hand, represent the world as a distribution of objects \varun{on a low dimensional manifold?} given the space of natural images, where each percept is a sample that it uses to model that distribution. As a result, CNN-based systems scale and generalize very well to new objects and instances, can accommodate diverse and noisy image data, and are fairly robust to unstructured environments. The distributions over all object classes and all images are very high dimensional \varun{over all object classes? This should be mapping not distribution} and very diverse, and as such each image-label pair represents very little of these distributions. As a result CNNs typically require thousands of examples of each object class it cares about, across millions of annotated image samples to achieve good performance \cite{zhou2017places}. This has been achievable in standard computer vision  tasks such as general image classification \cite{krizhevsky2012imagenet} \cite{szegedy2015going} \cite{he2015delving} and object detection \cite{ren2015faster} \cite{liu2016ssd} \cite{redmon2016you} in Internet images \varun{cite large scale datasets?}. 

%Developing reliable segmentation techniques for robot vision is integral for intelligent robots to reason about and interact with the commonplace environments such as homes, workplaces, and on roads. In computer vision, semantic segmentation has improved rapidly in the last few years with the use of convolutional neural networks, or CNNs. Despite these advances, semantic segmentation still faces two major challenges: representing distributions that classify every pixel in an image is much more difficult to model than classifying images or detecting  objects, and the cost of providing segmentation annotations is prohibitive for creating datasets at the scale required by CNNs to perform well on the task.

%Segmentation for robot vision is even more challenging since the research community has mostly focused on achieving state-of-the-art performance without constraints on model speed, using models with millions of parameters that require billions of operations to classify each image \cite{canziani2016analysis}. What's more, these models are trained on and evaluated using biased datasets composed of carefully chosen images \varun{this is a strong statement, citations?} and labeled with rigorous annotation processes. Robot vision requires more efficient CNN architectures for real-time performance, and the data provided is inherently noisy and uncurated as the datasets are often acquired while robots engage in tasks like navigating about a home. As a result, robots rarely benefit from training their perception systems exclusively with standard segmentation datasets, and even when it is applicable the computational constraints make it difficult to represent complex distributions.

% If you do not have a lot of images, as is often the case in segmentation, the primary way to create a network that can perform well on this task is \emph{transfer learning}.This means you first train your network on a different task that has a lot of labeled data, and because a model of $P(Y_new \vert X)$ is still learning what to look for in the space of all images to map it to some label Y, the parameters of this different task are very reusable, or transferable. The common method is to train first, or \emph{pretrain}, on ImageNet, a dataset of 1MM images that have a single classification for each image, and then retrain the parameters that output labels for your target task, or \emph{finetune}, using the smaller set of data actually associated with the target task. However, transfer learning can never outperform how well a CNN would perform on a task if you had enough data in your target task, only approach that performance.

% Therefore robot datasets made specifically for robot vision segmentation tasks are even smaller than their general counterparts, and often have so little labeled data that even with transfer learning they are poorly suited for data-driven vision solutions like CNN. 

% We believe that by pretraining a dataset with simulation data that is generated to be similar to the task data instead of by transferring from another task, compact data driven models can more effectively optimize for robot vision task with limited data. \varun{In this work, we show that given a specific task where limited training data is available, pretraining a CNN based model on simulated image data from a different domain but on a similar task, provides advantages compared to pretraining from an orthogonal visual task. Concretely, we demonstrate that a model pretrained on simulation segmentation data can better learn representations for performing semantic segmentation on new domains when the amount of annotated data from the new domain is low or is difficult/costly to acquire, when compared to a model pretrained on a different task, such as image classification.}

% The benefits of simulation have been used in other fields of computer vision besides real-time segmentation where supervision is even more difficult to attain. This is because in constructing the model with objects that themselves have class labels, the images sampled from these simulations can be automatically annotated. Scene flow, for example, where for each image in a video the vision model attempts to map each pixel to a vector in 3D space, is almost impossible to label any other way. Moreover, sampling from simulation for control over the amount of data in the dataset, and the diversity of that data


% However, in robotics it is often not enough to only know the label and position of the object in the image. For a robot to physically interact with objects and agents in an unstructured environment, it needs the ability to reason about the geometry and semantics of the environment in more generalizable fashion that is still real-time. CNNs have also yielded very promising results in extracting the geometry of object classes by learning to generate a masks of objects with semantic labels, also called semantic segmentation. However, most of the progress made in segmentation in the computer vision community does not run close to real time, using models that have hundreds of millions of parameters and require tens of gigaflops of calculations per image for inference \cite{canziani2016analysis}. 

% Another barrier to progress in segmentation is dataset size. While some image datasets for image classification have over of 1 million annotated images \cite{russakovsky2015imagenet}, the most comprehensive segmentation datasets have only tens of thousands of annotated frames in spite of being more complex learning problems. Canonical literature machine learning and pattern recognition in addition to the empirical successes of CNN-based solutions for computer vision problems with lots of data \cite{krizhevsky2012imagenet} shows that for complex problems, large datasets is important for solving the problem. The primary issue with creating large segmentation datasets is that the time required to annotate an image for segmentation is dramatically greater than for other vision tasks, sometimes taking as long as 90 minutes per frame on average \cite{richter2016playing}. These small datasets are especially an issue for robotics because as robotics data is usually not well regularized or class-balanced, noisy, and generally small and focused on a specific task, robotics approaches that use these data-driven models are often dependent on using large computer vision datasets to augment the model training process.

%Popular semantic segmentation datasets like  SUN3D \cite{xiao2013sun3d} and NYU RGB-D v2 \cite{Silberman:ECCV12}, where there are 5285 labeled frames for 37 classes and 1449 labeled frames for 13 classes respectively, do not have nearly enough annotated data for CNN-based approaches to find generalizable solutions to the the problem of semantic object segmentation. 

% Some datasets like MS-COCO \cite{lin2014microsoft} to reduce this time requirement by only annotating segments of particular objects in each frame instead of all of the objects in the image, and by using course annotations, but even these techniques result in datasets that a very long time to create and are in the tens of thousands. In addition, the annotation quality of such datasets can make these datasets not representative of the objects that robots encounter. However, datasets that do not segment the entire scene in each frame are often inappropriate for interactive robot applications and tasks like navigation, and obstacle avoidance where robots need to reason about the entire space. Furthermore, imperfect annotations can cause CNNs to have difficulty with getting results near object boundaries in the image and fail consistently on objects that are occluded or small. As a result, these datasets alone can be insufficient for training a model to perform segmentation for robots.


% In this work, we explore whether real-time CNN-based semantic segmentation approaches can be improved for robotics applications by augmenting the training process with large amounts of synthetically generated data before fine-tuning on the real data specific to the task. Large neural networks have a tendency to over-fit and take a long time to converge, and seminal empirical \cite{krizhevsky2012imagenet} \cite{he2015delving} and theoretical works \cite{bengio2009learning} \cite{glorot2010understanding} \cite{yosinski2014transferable} highlight the importance of data augmentation and weight initialization to avoid these shortcomings. Synthetic image data generated from simulated environments are well suited for augmenting the training process because of how realistic 3D rendering engines like VRay, Unreal Engine 4, and Unity 5, and video games like \textit{Grand Theft Auto V} and \textit{Mirror's Edge} have become, and because can be used to generate perfect annotations segmentations automatically or at an highly reduced rate. 

% We tested these ideas by conducting three experiments on our semantic segmentation architecture using a number of datasets that are both synthetic and real, and vary in size, content, and quality. We varied the dataset combinations and training techniques, and comparatively evaluated the resultant models on standard segmentation metrics to determine the most beneficial dataset combinations and training approaches. In the first experiment, we trained standard real datasets useful for indoor robots and autonomous cars using data-transformation augmentation techniques, transfer learning from ImageNet, and compare that to pretraining with synthetic semantic segmentation data. Our results show an average 13.4\% increase in segmentation performance by pretraining on synthetic data. In the second experiment we examine the degree of benefit of ``\textit{semantic domain similarity}", or the idea that augmenting training with synthetic data from a single semantic domain (e.g. autonomous driving) is better than using simply a diverse set of visual data, by pretraining the real autonomous car dataset on synthetic indoor data and the real indoor dataset on synthetic autonomous car data. Our results show that there is a notable average 10\% decrease in performance when real data is trained over a synthetic dataset that has low \textit{semantic domain similarity} and is similar in size to a synthetic dataset that has high \textit{semantic domain similarity}. However, we also noted that the model trained on real data and a synthetic dataset with low \textit{semantic domain similarity} but that is much larger than the dataset with high \textit{semantic domain similarity} outperformed the best model trained on a semantically similar dataset pair. In the last experiment, we captured a small amount of data from a robot designed not for visual data acquisition but for human robot interaction, annotated it without explicit adherence to any dataset's class list, and tested the degree of performance improvement these techniques afford semantic segmentation in a specific robot task.     

%% Related work
%This gap in efficiency only widens as batch size is increased, but that is less of a concern in robotics where each frame will be evaluated in real time.  

% MS-COCO \cite{lin2014microsoft}

% \subsection{Data Augmentation}
% Data augmentation for increasing the effectiveness of CNNs has been researched heavily since even before they gained popularity in computer vision \cite{sanchez2011high} \cite{ciregan2012multi} \cite{bengio2009learning}. Classic data augmentations use label-preserving transformations of the image and ground-truth label include scaling, rotations, flipping, random cropping, and color transformations, and for data sampled from video reconstructing the scene and re-sampling. However, these augmentations have been shown to have limited effectiveness \cite{Girshick_2014_CVPR}, and require close observation of the training process using early stopping to prevent over-fitting \cite{caruana2001overfitting}. The most effective and commonly utilized method for augmenting smaller datasets is \textit{curriculum learning} \cite{bengio2009curriculum}, which involves training a model architecture on similar, simpler data from one or more datasets before retraining this model using the smaller evaluation dataset, and \textit{transfer learning} \cite{yosinski2014transferable} \cite{oquab2014learning}, where a model that is pretrained on a different task and then the features are ``transferred" by taking the trained model, reinitializing the inference layers, and training only the inference layers. Transfer learning is so effective that at this point, with very general learning architectures like ResNet and VGG, it is standard practice to initialize these networks by pretraining them on ImageNet. However, the theory behind curriculum learning and transfer learning that we leverage indicates that there are potential gains by pretraining on data that is evaluated in the same way, as well as datasets that are larger and are more varied in their content. 




%% Justification
% In neural network theory, it has been shown that a multilayer full-connected feed-forward neural network structure and a nonlinear element can approximate any function given a number of parameters exponential in the size of the space of the function it is approximating \cite{kuurkova1992kolmogorov}. Specifically, for a two-layer network approximating a function in $n$ dimensions, the first layer having  $nm( m + 1 )$ units and the second having $m^2( m + 1 )^n$ units, network will approximate that function to a small real positive error $\epsilon$. Convolutional neural network are far more efficient than fully connected networks, but with this exponential upper bound, we assume that the number of parameters required to map a function is still exponential in the dimensionality of the space of the function. Assuming reasonably that $P_{i}(Y|X)$ and $P_{t}(Y|X)$ have similar dimensionality, given that their dimensionality will be dominated by $P(X)$, a large network of similar structure with more paramters will have exponentially more capacity more capacity

%pretraining is so effective and so ubiquitous in deep learning applications that standard learning architectures like ResNet and VGG are almost never trained from scratch, with most people opting to train their tasks using a model  already trained on ImageNet.

% This concept overlaps heavily in literature with data augmentation, or the idea that you can regularize bias in the network or increase the amount of unique inputs a deep network sees by preprocessing the input data. Data augmentation for increasing the effectiveness of neural networks researched heavily even before they gained popularity in computer vision \cite{sanchez2011high} \cite{ciregan2012multi} \cite{bengio2009learning}. Classic data augmentations use label-preserving transformations of the image and ground-truth label include scaling, rotations, flipping, random cropping, and color transformations, and for data sampled from video reconstructing the scene and re-sampling. However, these augmentations have been shown to have limited effectiveness \cite{Girshick_2014_CVPR}, and require close observation of the training process using early stopping to prevent over-fitting \cite{caruana2001overfitting}. 

%% Approach
% For our evaluations we considered a few different general network architectures: a fully convolutional ResNet-50 \cite{he2016deep}, SqueezeNet \cite{iandola2016squeezenet} modified with upsampling for segmentation, and ENet \cite{paszke2016enet}. VGG and ResNet have the advantage of already coming with ImageNet pretrained models and have been shown to generalize well to many problems, including segmentation, and are appropriate for applications like autonomous vehicles where power and compute resources are less constrained. However, for applications such as drones and household robots, optimizations are necessary, and the optimizations that we tried did not substantially speed up training, and preliminary tests did appear to lower the performance. SqueezeNet has much promise as a lightweight optimized model. However, the fully convolutional AlexNet in Long \etal \cite{long2015fully} showed relatively poor segmentation performance. Taking design cues from the modules that distinguished both ResNets GoogLeNet \cite{szegedy2015going}, and being designed from the beginning for efficient semantic segmentation, ENet was the best choice for our task.


